On Non-Interactive Source Simulation via Fourier Transform

The non-interactive source simulation (NISS) scenario is considered. In this scenario, a pair of distributed agents, Alice and Bob, observe a distributed binary memoryless source $(X^d,Y^d)$ generated based on joint distribution $P_{X,Y}$. The agents wish to produce a pair of discrete random variables $(U_d,V_d)$ with joint distribution $P_{U_d,V_d}$, such that $P_{U_d,V_d}$ converges in total variation distance to a target distribution $Q_{U,V}$ as the input blocklength $d$ is taken to be asymptotically large. Inner and outer bounds are obtained on the set of distributions $Q_{U,V}$ which can be produced given an input distribution $P_{X,Y}$. To this end, a bijective mapping from the set of distributions $Q_{U,V}$ to a union of star-convex sets is provided. By leveraging proof techniques from discrete Fourier analysis along with a novel randomized rounding technique, inner and outer bounds are derived for each of these star-convex sets, and by inverting the aforementioned bijective mapping, necessary and sufficient conditions on $Q_{U,V}$ and $P_{X,Y}$ are provided under which $Q_{U,V}$ can be produced from $P_{X,Y}$. The bounds are applicable in NISS scenarios where the output alphabets $\mathcal{U}$ and $\mathcal{V}$ have arbitrary finite size. In case of binary output alphabets, the outer-bound recovers the previously best-known outer-bound.

==> Fourier.tex <==
\subsection{Boolean Fourier expansion on product probability spaces}
We start with a brief overview of the well-known Fourier expansion on Boolean cube \citep{ODonnell2014,Wolf2008} that has applications in computational learning \citep{blais2010polynomial,Mossel_ODonnell,mossel2004learning,furst1991improved,Heidari_ISIT19}. 


Let $\bfX = (X_1, X_2, ..., X_d)$ be a vector of mutually independent random variables taking values from a subset $\mathcal{X}\subset \RR^d$.  Let $\mu_j$ and $\sigma_j$ be the mean and standard-deviation of $X_j, j\in [d]$. Suppose that these random variables are non-trivial, that is $\sigma_j>0$ for all $j\in [d]$. The Fourier expansion is defined via a set of basis functions called \textit{parities}. 
The \textit{parity} for a subset $\mathcal{S}\subseteq [d]$ is defined as  $$\pS(\bfx)\deq \prod_{i\in \mathcal{S}}\frac{x_i-\mu_i}{\sigma_i},\qquad  \text{for all}~ \bfx \in \RR^d.$$ Since $X_i$'s are mutually independent, the parities are orthonormal, that is $\EE[ \pS(\bfX)^2]=1$ for any subset $\mathcal{S}$, and $\EE[\pS(\bfX)~ \pset{\mathcal{T}}(\bfX)]=0$ when $\mathcal{T}\neq \mathcal{S}$ (that is $\exists x\in \mathcal{T}\medcup \mathcal{S}$ such that $x\notin \mathcal{T}\medcap \mathcal{S}$). Under the assumption that $\mathcal{X}=\pmm^d$, the parities form an orthonormal basis for the space of bounded functions \citep[Theorem 1.1]{ODonnell2014}. That is, any bounded function $f:\pmm^d\mapsto \RR$ can be written as a linear combination of the form
 $$f(\bfx)=\sum_{\mathcal{S}\subseteq [d]} \fS~\ps(\bfx), \quad \text{for all}~ \bfx \in \pmm^d,$$
  where $\fS\in \RR$ are called the {\it Fourier coefficients} of $f$ with respect to $D_{\bfX}$, the distribution of $\bfX$.  Further, the Fourier coefficients can be computed as  $\fS= \EE[f(\bfX)\pS(\bfX)]$, for all subsets $\mathcal{S}\subseteq [d]$.
%For that, we propose a method to make the parities orthogonal.   and exist a number of redundant features. In this section, we develop a method based on our Fourier framework to detect and remove redundant features. 
%


%In this section, we develop a new Fourier expansion for function of arbitrarily correlated features. For that, we propose a method to make the parities orthogonal. 
\subsection{Orthogonalization}

We proceed by constructing a Fourier expansion for functions of correlated random variables. Note that, in a general probability space with correlated features, the standard Fourier expansion is no longer well-defined. Because the parities $\pS$ are not necessarily orthogonal. That said, we construct our Fourier expansion by adopting a Gram-Schmidt-type procedure to make the parities \textit{orthogonal}. Then, we use this basis to develop our Fourier expansion for functions of correlated random variables. Based on that, we establish the following result.  


\begin{proposition}[\textbf{Correlated Fourier Expansion}]\label{prop:Fourier_correlated}
Let  $D_{\bfX}$ be any probability distribution on $\pmm^d$. Then  there are a set of orthonormal parity functions $\ptS, \mathcal{S}\subseteq [d]$ such that 
any bounded function $g:\pmm^d\mapsto \RR$ is decomposed as
$$g(\bfx)=\sum_{\mathcal{S}\subseteq [d]} \gtS \ptS(\bfx),$$
for all $\bfx\in \pmm^d$ except a measure-zero subset. Further, the coefficients $\gtS$ are unique and obtained from $\gtS=\EE[g(\bfX)\ptS(\bfX)]$.
%  Let $\ptS$'s be the orthogonalized parities as defined in \eqref{eq:GramSchmidt}. Then, for all $\bfx\in \pmm^d$ except a measure-zero subset, $f(\bfx)$ is decomposed as  $f(\bfx)=\sum_{\mathcal{S}\subseteq [d]} \ftS \ptS(\bfx),$ where the summation is taken over all $\mathcal{S}\subseteq [d]$ for which $\ptS$ is not trivial. Further, the coefficients $\ftS$ are unique and obtained from $\ftS=\EE[f(\bfX)\ptS(\bfX)]$.
\end{proposition}
%\begin{proposition}[\textbf{Correlated Fourier Expansion}]\label{prop:Fourier_correlated}
%Let  $P_{\bfX}$ be any probability distribution on $\pmm^d$ and $f:\pmm^d\mapsto \RR$ be a bounded function. Let $\ptS$'s be the orthogonalized parities as defined in \eqref{eq:GramSchmidt}. Then, for all $\bfx\in \pmm^d$ except a measure-zero subset, $f(\bfx)$ is decomposed as  $f(\bfx)=\sum_{\mathcal{S}\subseteq [d]} \ftS \ptS(\bfx),$ where the summation is taken over all $\mathcal{S}\subseteq [d]$ for which $\ptS$ is not trivial. Further, the coefficients $\ftS$ are unique and obtained from $\ftS=\EE[f(\bfX)\ptS(\bfX)]$.
%\end{proposition}

\begin{proof}
Let $\mu_j$ and $\sigma_j$ be the mean and standard deviation of each input random variable $X_j, j\in [d]$. Suppose that these random variables are non-trivial, that is $\sigma_j>0$ for all $j\in [d]$. The proof is based on an orthogonalization process that is explained in the following.

\noindent\textbf{Orthogonalization process:}
%Assume that the features $X_1, X_2, ..., X_d$ are generated according to an arbitrary joint probability distribution $P_{\bfX}$. Here, the features can be arbitrary real-valued random variables. 
Fix the following ordering for subsets of $[d]$: 
\begin{align}\label{eq:subset_ordering}
\emptyset, \{1\}, \{2\}, \{1, 2\}, \{3\}, \{1, 3\}, \{2, 3\}, \{1, 2, 3\}, \cdots, \{1, 2, ..., d\}.
\end{align}
%Let $\mathcal{S}_1, \mathcal{S}_2, ..., \mathcal{S}_{2^d}$ be all the subsets of $[d]$. 
 We apply the Gram-Schmidt process on  $\pSi$ with the above ordering. 
 The first orthogonalized parity is trivially given by $\ptset{\emptyset}\equiv 1$. 
%  The first orthogonalized parity is the identity function, that is  $\psi^{\circ}_{\emptyset}(\bfX)\deq 1$ for all $\bfX\in \RR^d$. Then, 
The orthogonalized parity  corresponding to the $i$th subset is obtained from the following operation:
%\vspace{-10pt}
\begin{align}\nonumber
 \ptildSi&\equiv \pSi- \sum_{j=1}^{i-1} \<\ptSj,\pSi\> ~ \ptSj,\\\label{eq:GramSchmidt}
  \ptSi &\equiv \left\{ \begin{array}{ll}
 \frac{\ptildSi}{\norm{\ptildSi}_2} & \text{if}~ \norm{\ptildSi}_2>0,\\
  0 & \text{otherwise.}
 \end{array}  \right.
 \end{align}
where $\norm{\ptildSi}_2 = \sqrt{\<\ptildSi,\ptildSi\>}$. 
By construction, the resulted nontrivial parities $\ptSi$'s are orthonormal, that is $\<\ptSi, \ptSj\>=0$ for $i\neq j$ and $\<\ptSi, \ptSi\>=1$ if $\ptSi$ is not trivial. The rest of the argument, given in Appendix \ref{appx:prop_Fourier_correlated},
 follows by showing that $\ptS$'s span the space of all bounded functions.  
\end{proof}


==> Notations_Mohsen.tex <==
%========================================================================================
%------------------------- This header contains shorthands and notations ----------------
%========================================================================================
\newcommand{\optfont}[1]{\mathsf{#1}}
\newcommand{\prodin}{\prod_{i=1}^n}
\newcommand{\sumin}{\sum_{i=1}^n}

%====================== double script fonts  =====================================

\global\long\def\RR{\mathbb{R}}
\global\long\def\CC{\mathbb{C}}
\global\long\def\NN{\mathbb{N}}
\global\long\def\QQ{\mathbb{Q}}
\global\long\def\ZZ{\mathbb{Z}}
\global\long\def\EE{\mathbb{E}}
\global\long\def\PP{\mathbb{P}}
\global\long\def\FF{\mathbb{F}}
\global\long\def\11{\mathbbm{1}}

%====================== math bold fonts  =====================================

\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

\newcommand{\clJ}{\mathcal{J}}
\newcommand{\clU}{\mathcal{U}}
\newcommand{\clV}{\mathcal{V}}
\newcommand{\clX}{\mathcal{X}}
\newcommand{\clY}{\mathcal{Y}}


%====================== shortcuts for operators  =====================================

\global\long\def\+{\oplus}
\global\long\def\P{\mathsf{P}}
\global\long\def\dd{\cdots}
\newcommand\pmm{\{-1,1\}}


\def\var{\optfont{var}}

\newcommand{\prob}[1]{\PP\Big\{  #1 \Big\} }
\def\<{\langle}
\def\>{\rangle}

\newcommand{\sign}{\mathsf{sign}}
\newcommand{\OR}{\mathsf{OR}}
\newcommand{\AND}{\mathsf{AND}}
\newcommand{\MAJ}{\mathsf{MAJ}}

\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\norm}[1]{\lVert#1\rVert}


\newcommand*{\medcap}{\mathbin{\scalebox{1}{\ensuremath{\bigcap}}}}%
\newcommand*{\medcup}{\mathbin{\scalebox{1}{\ensuremath{\bigcup}}}}%
\newcommand*{\medprod}{\mathbin{\scalebox{1}{\ensuremath{\prod}}}}%

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%-------- delta = for definition -----
\usepackage{stackengine}
\def\deq{\mathrel{\ensurestackMath{\stackon[1pt]{=}{\scriptstyle\Delta}}}}

%===============================================================================
%------------------------- Special Notations -----------------------------------
%===============================================================================

%++++++++++++++++++++++++   Original Symbls ++++++++++++++++++++++++++++++++++++

\def\fS{\mathtt{f}_{\mathcal{S}}}
\def\fSi{\mathtt{f}_{\mathcal{S}_i}}
\def\fSj{\mathtt{f}_{\mathcal{S}_j}}

\def\ftS{{f}_{\mathcal{S}}}
\def\ftSi{{f}_{\mathcal{S}_i}}
\def\ftSj{{f}_{\mathcal{S}_j}}

\def\fJ{{\mathtt{f}}^{\subseteq \mathcal{J}}}
\def\ftJ{{f}^{\subseteq \mathcal{J}}}
\newcommand\ftsubset[1]{{f}^{\subseteq #1}}


\def\ftJstar{{f}^{\subseteq {\mathcal{J}^*}}}
\def\hJ{h_{\mathcal{J}}}

\def\gS{{g}_{\mathcal{S}}}
\def\gtS{{g}_{\mathcal{S}}}

\def\gJ{g^{\subseteq J}}

\def\ps{\phi_\mathcal{S}}
\def\pS{\ps}
\def\pSi{\phi_{\mathcal{S}_i}}
\def\pSj{\phi_{\mathcal{S}_j}}
\newcommand{\pset}[1]{{\phi}_{#1}}

\def\ptS{{\psi}_\mathcal{S}}
\def\ptSi{{\psi}_{\mathcal{S}_i}}
\def\ptSj{{\psi}_{\mathcal{S}_j}}
\newcommand{\ptset}[1]{{\psi}_{#1}}

\def\ptildS{\tilde{\psi}_\mathcal{S}}
\def\ptildSi{\tilde{\psi}_{\mathcal{S}_i}}
\def\ptildSj{\tilde{\psi}_{\mathcal{S}_j}}
\newcommand{\ptildset}[1]{\tilde{\psi}_{#1}}





%++++++++++++++++++++++++   Esimation Symbls ++++++++++++++++++++++++++++++++++++
\def\festS{\hat{\mathtt{f}}_{ S} }
\def\festSi{\hat{\mathtt{f}}_{\mathcal{S}_i}}
\def\festSj{\hat{\mathtt{f}}_{\mathcal{S}_j}}



\def\festJ{\hat{\mathtt{f}}^{\subseteq \mathcal{J}}}
\def\festtJ{\hat{{f}}^{\subseteq \mathcal{J}}}


\def\fbarS{\bar{f}_{ S} }
\def\fbarJ{\bar{f}^{\subseteq \mathcal{J}}}


\def\festtS{\hat{f}_{\mathcal{S}}}
\def\festtSi{\hat{f}_{\mathcal{S}_i}}
\def\festtSj{\hat{f}_{\mathcal{S}_j}}




%\def\FestS{\hat{\mathsf{F}}_{S} }
\def\FestS{\festS}

%\def\FestJ{\hat{\mathsf{F}}^{\subseteq \mathcal{J}}}
\def\FestJ{\festJ}

\def\FestSone{\hat{f}_{(1), S} }
\def\FestJone{\hat{f}_{(1)}^{\subseteq \mathcal{J}}}
\def\FestJi{\hat{f}_{(i)}^{\subseteq \mathcal{J}}}
\def\FJibar{\bar{f}_{(i)}^{\subseteq \mathcal{J}}}
\def\FJonebar{\bar{f}_{(1)}^{\subseteq \mathcal{J}}}
\def\FSonebar{\bar{f}_{(1), S} }

\def\pestS{\widehat{\phi}_{\mathcal{S}}}
\def\pesttS{\widehat{\psi}_\mathcal{S}}
\newcommand\pestsubset[1]{\widehat{\psi}_{#1}}
\def\PestS{\widehat{\Psi}_{\mathcal{S}}}





%++++++++++++++++++++++++   Algorithm Symbls ++++++++++++++++++++++++++++++++++++

\def\Jalg{\hat{\mathcal{J}}_n}
\def\falg{\hat{f}^{\subseteq \Jalg}}
\def\fJalg{{f}^{\subseteq \Jalg}}

\def\predict{\hat{g}}
\def\Peg{P_e(\predict)}


\def\Jalgb{\hat{\mathcal{J}}_2}
\def\falgb{\hat{f}^{\subseteq \Jalgb}}
\def\fJalgb{{f}^{\subseteq \Jalgb}}
\def\predictb{\hat{g}_2}





\def\rndJalg{\mathscr{J}_{alg1}}
\def\rndfalg{\mathsf{F}_{est}^{\subseteq \rndJalg}}
\def\rndpredict{\mathsf{G}_{alg1}}
\def\frndJalg{{f}^{\subseteq \rndJalg}}



%\newcommand{\barf}{\bar{f}}
 %\def\fbarJ{\bar{f}^{\subseteq J}}
\def\fJbar{f^{\subseteq \bar{J}}}
%\def\fbarJbar{\bar{f}^{\subseteq \bar{J}}}
%\def\festJbar{{f}_{est}^{\subseteq \bar{J}}}
%\def\fbarS{\bar{f}_{S} }
%\def\funivJbstar{{f}_{unv}^{\subseteq {\bar{J}^*}}}
%\def\funivJ{{f}_{unv}^{\subseteq {J}}}
%\def\Je{\mathcal{J}_{\mathbf{e}}}
%\def\E_mu{\mathcal{E}(\epsilon')}


\def\L2{\mathcal{L}^2(\mathcal{X}, P_{\bfX})}
\def\Pspace{(\mathcal{X},P_{\bfX})}





\newcommand{\Pek}{P_{opt}(k)}

\def\mone{M_n}
\def\monebar{\overline{M}_n}
\def\score{\mone}
\def\imscore{\mone}


\def\mtwo{M_n^{(2)}}

\def\E_mu{\mathcal{E}_{\mu}(\epsilon')}
\def\empD{\hat{D}_n}
\def\empLoss{L_{\empD}}
\def\Loss{L_D}
\def\optempLoss{L^*_{\empD}}
\def\optLoss{L^*_D}
\def\empftJ{\festtJ}


\def\Piest{\hat{\Pi}_Y}
\def\Piy{\Pi_Y}
\def\Pibar{\bar{\Pi}_Y}
\def\PiJ{\Pi_Y^{\mathcal{J}}}
